Interlacing Families II: Mixed Characteristic Polynomials and the Kadison-Singer Problem

We use the method of interlacing families of polynomials introduced to prove two theorems known to imply a positive solution to the Kadison--Singer problem. The first is Weaver's conjecture $KS_{2}$ \cite{weaver}, which is known to imply Kadison--Singer via a projection paving conjecture of Akemann and Anderson. The second is a formulation due to Casazza, et al., of Anderson's original paving conjecture(s), for which we are able to compute explicit paving bounds. The proof involves an analysis of the largest roots of a family of polynomials that we call the "mixed characteristic polynomials" of a collection of matrices.

==> kshistory.tex <==
\section{History}\label{sec:history}

In their 1959 paper, Kadison and Singer \cite{orig_ks} posed a fundamental question that arose in the formalization of quantum mechanics using $C^{*}$--algebras.
Let $\mathcal{H}$ be a complex, separable Hilbert space and let $\mathcal{B}(\mathcal{H})$ be the space of bounded linear transformations on $\mathcal{H}$.
\begin{question}
Does every pure state on the algebra of diagonal operators on
$\ell_2(\mathbb{N})$ extend
  uniquely to a pure state on the algebra of all bounded operators on $\ell_2$?
\end{question}

The case when $\mathcal{B}(\mathcal{H}) = \ell^\infty(\N)$ has become known as the {\em Kadison--Singer problem}.  (Despite an indication in the original paper that they felt the answer was negative, Kadison and Singer did not formally conjecture either way).

In the original paper, Kadison and Singer noted that the resolution of their question was equivalent to a question regarding pavings of operators in $\ell^\infty(\N)$.
A {\em paving} of an operator $M$ with respect to a partition $\pi_1, \dots, \pi_r$ of its basis is the sum of the projections of $M$ onto the parts of the partition.
The first progress on resolving the question occurred 20 years later when Anderson showed that the Kadison--Singer problem was equivalent to a question regarding pavings of finite operators \cite{anderson1979a}.
This led to a series of problems that are collectively known as the {\em Anderson Paving Problems}, an example of which is the following:
\begin{question}[Anderson Paving]\label{anderson_paving_question}
Given $n > 0, \epsilon > 0$ and $M$ an $n \times n$ matrix with $0$ diagonal and $\norm{T} \leq 1$, does there exist a partition of 
$\{1, \dots, n\}$ into $r = r(\epsilon)$ sets $A_1, \dots, A_r$ such that
\[
\norm{P_{A_j}TP_{A_j}} \leq \epsilon
\]
for all $j$ (where $P_{A_j}$ is the projection operator onto the coordinates in $A_j$)?
\end{question}
%We should point out that all of the equivalences required there being a {\em uniform} bound on $r$ (that is, independent of $n$).

Anderson's papers  \cite{anderson1979a, anderson1979b, anderson1981} drew an increased interest to the problem and resulted in a number of papers on the subject.
In particular, it was discovered that similar questions from a number of different fields were equivalent to the Kadison--Singer problem, including
Akemann and Anderson's projection paving conjecture \cite{akemann1991lyapunov},
Weaver's discrepancy theoretic $KS_{r}$ and $KS_{r}'$ conjectures \cite{weaver},
the Bourgain--Tzafriri Conjecture \cite{BTKS,casazza2006kadison}, and
the Feichtinger Conjecture and the $R_{\epsilon}$-Conjecture \cite{casazza2005frames}.
Other restrictions of the original problem were proved to be true, including ones by Tropp \cite{Tropp2007}, Popa \cite{Popa2013}, Lawton \cite{Lawton2010}, Paulsen \cite{Paulsen2008}, Akemann et al. \cite{akemann2012kadison}, Halpern et al. \cite{halpern1985matrix}, and Baranov and Dyakonov \cite{BarDya2010}. 
We refer the reader to \cite{AIM} for more information on equivalences and partial results.

For a more detailed discussion of the history of the Kadison--Singer problem and a host of other related conjectures, we refer the reader to \cite{casazza2006detailed}.


==> ksintro-scratch.tex <==
\section{Introduction}\label{sec:outline}
In 1959, Kadison and Singer posed the following fundamental question in operator
  theory: 
\begin{question}[Kadison-Singer Problem] \label{question:ks} Does every pure state on the (abelian)
von Neumann algebra $\mathbb{D}$ of bounded diagonal operators on
$\ell_2$ have a unique extension to a pure state on $B(\ell_2)$, the
von Neumann algebra of all bounded operators on $\ell_2$?
\end{question}
Recall that a state on a von Neumann algebra is a positive linear functional
  which maps the identity to $1$, and a pure state is an extreme point of the
  (convex) set of all states.
Though they did not formally conjecture either way, they suspected a negative
  answer to their question.

Beginning with the work of Anderson in 1979, a positive resolution to Question \ref{question:ks} was 
  shown to be equivalent to several elementary conjectures about finite complex matrices.
Among them are the following.
\begin{conjecture}[Anderson Paving] For every $\epsilon>0$ there is an
$r\in\mathbb{N}$ such that for every $n\times n$ complex matrix $T$ with zero
diagonal, there are coordinate projections $P_1,\ldots,P_r$ with $\sum_{i=1}^r P_i=I$ such that
$$ \|P_iTP_i\|\le \epsilon\|T\|\qquad\textrm{for $i=1,\ldots,k$}.$$
\end{conjecture}

Our first result resolves a discrepancy theoretic conjecture on complex vector spaces due to Weaver \cite{weaver}.
\begin{theorem}\label{thm:weaver}
Let $w_{1}, \dots , w_{m} \in \Complex{d}$ satisfy $\norm{w_{i}} \leq 1$ for all $i$
  and suppose
\[
\sum_{i=1}^m \abs{\langle u, w_{i} \rangle}^{2} = 18
\]
for every unit vector $u \in \Complex{d}$. 
Then there exists a partition $S_{1}, S_{2}$ of $\setof{1, \dots , m}$ so that
\[
\sum_{i \in S_1} \abs{\langle u, w_{i} \rangle}^{2} \leq  16
\qquad
\text{and}
\qquad
\sum_{i \in S_2} \abs{\langle u, w_{i} \rangle}^{2} \leq  16
\]
for every unit vector $u \in \Complex{d}$.
\end{theorem}

The proofs of these theorems (as well as the statements of the respective conjectures) appear in Section~\ref{sec:theorems}.
They rely on our main technical result, which concerns collections of independently distributed random vectors.
We state it here, but defer the proof to the end of Section~\ref{sec:barrier}.

\begin{theorem}\label{thm:general}
Let $\epsilon > 0$ and let
  $v_1, \dots, v_m$ be independent random vectors in $\C^d$ with finite support such that 
\begin{equation}\label{eqn:mainSum}
\sum_{i=1}^m \expec{}{v_{i} v_{i}^{*}} = I_d,
\end{equation}
and
\[
\expec{}{ \norm{v_{i}}^{2}} \leq \epsilon, \text{for all $i$.}
\]
Then 
\[
\prob{}{ \norm{\sum_{i=1}^m v_i v_i^{*}} \leq (1 + \sqrt{\epsilon})^2 } > 0
\]
\end{theorem}

Theorem~\ref{thm:general} may be compared to the concentration inequalities of 
  Rudelson \cite{RudelsonIsotropic} and Ahlswede and Winter \cite{AhlswedeWinter}, which imply in
  our setting that $\|\sum_{i=1}^mv_iv_i^*\|^2 \leq C(\epsilon)\cdot\log d$ with high
  probability.
Here we are able to control the deviation at the much smaller
  scale $(1+\sqrt{\epsilon})^2$, but only with nonzero probability.

We will prove Theorem~\ref{thm:general} using the ``method of interlacing families of polynomials'' first introduced in \cite{lifts_paper}.
Section~\ref{sec:interlacing} will contain a review of interlacing polynomials along with some results from linear algebra and polynomial theory that we will need as tools in later proofs.

For our purpose, interlacing families of polynomials have the property that
  they always contain at least one polynomial whose largest root is at most the
  largest root of the sum of the polynomials in the family.
In Section~\ref{sec:mixed}, we prove that the characteristic polynomials of the matrices
  that arise in Theorem~\ref{thm:general} are such a family.
This proof requires us to consider the expected characteristic polynomials
  of certain sums of independent rank-$1$ positive semidefinite Hermitian matrices.
We call such an expected polynomial a \textit{mixed characteristic polynomial}.
To prove that the polynomials that arise in our proof are an interlacing family,
  we show that all mixed characteristic polynomials are real rooted.
Inspired by 
  Borcea and \Branden's proof of Johnson's Conjecture~\cite{BBjohnson},
  we do this by constructing multivariate real stable polynomials,
  and then applying operators that preserve real stability
  until we obtain the (univariate) mixed characteristic polynomials.

We then need to bound the largest root of the expected characteristic polynomial.
We do this in Section~\ref{sec:barrier} through a multivariate generalization of the barrier function argument
  of Batson, Spielman, and Srivastava~\cite{BSS}.
The original argument essentially considers the behavior of the roots
  of a real rooted univariate polynomial $p(x)$ under the operator
  $1 - \partial_{x}$.
It works by keeping track of an upper bound on the roots of the polynomial,
  along with a measure of how far above the roots this upper bound is.

In our multivariate generalization, we consider a vector $x$ to be {\em above
  the roots} of a real stable multivariate polynomial $p(x_1,\ldots,x_m)$ if
  $p(y_{1}, \dots , y_{m})$ is non-zero
  for every vector $y$ that is at least as big as $x$ in every coordinate.
The value of our multivariate barrier function at $x$ is the vector of the univariate
  barrier functions obtained by restricting to each coordinate.
We then show that we are able to control the values of the barrier function when operators
  of the form 
  $1 - \partial_{x_{i}}$
  are applied to the polynomial.  
Our proof is inspired by the methods used by Gurvits to prove an elegant strengthening of van der Waerden's conjecture on the minimum number of perfect matchings in a $k$-regular bipartite graph \cite{gurvitsOne}.
Gurvits's proof examines a sequence of polynomials similar to those we construct in our proof, and amounts to proving a lower bound on the constant term of the mixed characteristic polynomial.


==> kstheorems.tex <==
%\documentclass[11pt]{article}
%%\usepackage{amsmath,amsfonts,amsthm,amssymb,ifthen}
%\usepackage{amsmath,amsfonts,amsthm,amssymb,color}
%
%\textheight 8.5in
%\topmargin -0.2in
%\oddsidemargin 0.20in
%\textwidth 6.3in
%
%
%\input{defs}
%
%
%\begin{document}

\section{Proving the Theorems}\label{sec:theorems}

We begin by proving a theorem that seems to be useful in its own right, and then use it to give proofs of Theorem~\ref{thm:weaver} and Theorem~\ref{thm:anderson}.
\begin{theorem}\label{thm:partition}
Let $r > 0$ be an integer, and let $u_1, \dots, u_m \in \C^d$ be vectors such that $\norm{u_i}^2 \leq \delta$ for all $i$.
Then there exists a partition $\{ A_1, \dots A_r \}$ of $[m]$ such that 
\[
\norm{ \sum_{i \in A_j} {u_i} {u_i}^{*}} \leq \left(\frac{1}{\sqrt{r}}+\sqrt{\delta}\right)^{2}
\]
\end{theorem}
\begin{proof}
For each $i \in [m]$ and $k \in [r]$, define $w_{i,k} \in \C^{rd}$ to be the direct sum of $r$ vectors from $\C^d$, all of which are $0^d$ (the $0$-vector in $\C^d$) except for the $k^{th}$ one (which is a copy of $u_i$).
Now let $v_1, \dots, v_m$ be independent random vectors such that $v_i$ takes the values $\{ \sqrt{r} w_{i,k} \}_{k=1}^r$ each with probability $1/r$.

These vectors satisfy
\[
  \expec{}{v_{i} v_{i}^{*}}
= 
\begin{pmatrix}
u_{i} u_{i}^{*} & 0_{d \times d} & \dots & 0_{d \times d} \\
0_{d \times d} & u_{i} u_{i}^{*} & \dots & 0_{d \times d} \\
\vdots &  & \ddots &  \vdots \\
0_{d \times d} & 0_{d \times d} & \dots & u_{i} u_{i}^{*},
\end{pmatrix}
\quad \text{and} \quad 
\norm{v_{i}}^{2} = r \norm{u_{i}}^{2} \leq r \delta.
\]
So,
\[
\sum_{i=1}^m  \expec{}{v_{i} v_{i}^{*}} = I_{rd}
\]
and we can apply Theorem~\ref{thm:general} with $\epsilon  = r \delta$ to show that 
  there exists an assignment of each $v_i$ so that  
\[
\norm{
\sum_{k=1}^r
\sum_{i : v_i = w_{i,k}}
\left(\sqrt{r} w_{i,k} \right)
\left(\sqrt{r} w_{i,k} \right)^{*}
}
\leq (1+\sqrt{r \delta})^{2}.
\]
Setting $A_{k} = \{ i : v_i = w_{i,k} \}$ implies that 
\[
\norm{\sum_{i \in A_k} {u_i} {u_i}^{*}} 
= 
\norm{\sum_{i \in A_k} {w_{i,k}} {w_{i,k}}^{*}} 
\leq  
\frac{1}{r}
\norm{
\sum_{k=1}^r
\sum_{i : v_i = w_{i,k}}
\left(\sqrt{r} w_{i,k} \right)
\left(\sqrt{r} w_{i,k}\right)^{*}
}
\leq \left(\frac{1}{\sqrt{r}}+\sqrt{\delta}\right)^{2}.
\]
and this is true for all $k$.
\end{proof}

\subsection{$KS_2$}

The following conjecture is due to Weaver, as amended by \cite[Theorem 2]{weaver}.
It was shown in \cite{weaver} to imply a positive solution to the Kadison--Singer problem.

\begin{conjecture}\label{conj:weaver}
There exist universal constants $\eta \geq 2$ and $\theta > 0$ such that following is true:
Let $w_{1}, \dots , w_{m} \in \Complex{d}$ satisfy $\norm{w_{i}} \leq 1$ for all $i$
  and suppose
\begin{equation}\label{eqn:weaverCond}
  \sum_{i=1}^m \abs{\langle u, w_{i} \rangle}^{2} = \eta
\end{equation}
for every unit vector $u \in \Complex{d}$. 
Then there exists a partition $S_{1}, S_{2}$ of $\setof{1, \dots , m}$
  so that
\begin{equation}\label{eqn:weaverNeed}
  \sum_{i \in S_{j}} \abs{\langle u, w_{i} \rangle}^{2} \leq \eta - \theta,
\end{equation}
for every unit vector $u \in \Complex{d}$ and each $j \in \setof{1,2}$.
\end{conjecture}

A direct application of Theorem~\ref{thm:partition} shows the following strong version of Conjecture~\ref{conj:weaver}.

\begin{corollary}\label{cor:weaver}
Let $u_{1}, \dots , u_{m}$ be column vectors in $\Complex{d}$ such that
  $\sum_{i} u_{i} u_{i}^{*} = I$ and
  $\norm{u_{i}}^{2} \leq \alpha $ for all $i$.
Then, there exists a partition of $\setof{1,\dots ,m}$ into sets $S_{1}$
  and $S_{2}$ so that for $j \in \setof{1,2}$,
\begin{equation}\label{eqn:weaverStrong}
\norm{\sum_{i \in S_{j}} u_{i} u_{i}^{*}}
\leq 
\frac{(1+\sqrt{2 \alpha})^{2}}{2}.
\end{equation}
\end{corollary}
\begin{proof}
Set $r = 2$ and $\delta = \alpha$ in Theorem~\ref{thm:general}.
\end{proof}

Setting $\alpha = 1/18$ gives $\eta = 18$ and $\theta = 2$ for Theorem~\ref{thm:weaver}.

\subsection{Anderson Paving}

It was noted in Section~\ref{sec:history} that, while a proof of Weaver's $KS_2$ was sufficient for resolving the Kadison--Singer problem, paving (and therefore explicit paving bounds) seem to be of independent interest.  
Recall that $\mathcal{B}(\ell^\infty)$ is the collection of bounded linear functionals on $\ell^\infty$.
For an operator $T \in \mathcal{B}(\ell^\infty)$, let $E(T)$ be the {\em diagonalization of $T$}
\[
\langle E(T)e_i, e_j \rangle = 
\left\{
\begin{array}{rl}
\langle T e_i , e_i \rangle & \text{for } i = j \\
0 & \text{otherwise}
\end{array}\right.
\]
For a set $S \subseteq \N$, let $P_S$ be the projection operator
\[
\langle P_S e_i, e_j \rangle = 
\left\{
\begin{array}{rl}
1 & \text{for } i = j \in S \\
0 & \text{otherwise}
\end{array}\right.
\]
One version of Anderson's Paving Conjecture is the following:
\begin{conjecture}[Anderson Paving Conjecture]
For every $\epsilon > 0$, there exists an integer $r>0$ such that for every self--adjoint operator $T \in \mathcal{B}(\ell^\infty)$ with $E(T) = 0$, there exists a partition $\{ A_1, \dots, A_r \}$ of $\N$ such that 
\[
\norm{P_{A_i} T P_{A_i}} \leq \epsilon \norm{T}
\]
for all $i \in [r]$.
\end{conjecture}

%CEKP07 = 
%Pete Casazza, Dan Edidin, Deepti Kalra, and Vern I. Paulsen. Projections and the
%Kadison-Singer problem. Operators and Matrices, 1(3):391–408, 2007.

Employing arguments in \cite{CEKP07}, Harvey showed the following:
\begin{theorem}[Theorem~6.3 in \cite{harvey}]\label{thm:harvey}
The following are equivalent:
\begin{enumerate}
\item Anderson's paving conjecture is true
\item For all $\epsilon > 0$ and even integers $N \geq 2$, there exists an integer $r \geq 2$ such that for all integers $d > 0$ and all collections of vectors $u_1, \dots, u_m \in \C^d$ satisfying
\[
\sum_{i = 1}^m u_i u_i^* = I_d \qquad\text{and} \qquad \| u_i \|^2 \leq \frac{1}{N}
\]
for all $i$, there exists a partition $\{A_1, \dots, A_r \}$ of $[m]$ for which
\[
\norm{\sum_{i \in A_j} u_i u_i ^*} \leq \frac{1 + \epsilon}{N}
\]
for all $j \in [r]$.
\end{enumerate}
\end{theorem}
Moreover, the proofs in \cite{harvey} give explicit reductions and so specific values of $\epsilon, N, r$ can be propagated to specific paving bounds. 
Using Theorem~\ref{thm:general}, we are able to give a direct proof of the second statement listed in the the theorem above.
In the proof given, we optimize the value of $r$, but this can be adjusted for cases where the value of $\epsilon$ is the important one.

\begin{corollary}
The second statement in Theorem~\ref{thm:harvey} is true for any $r$ satisfying
\[
r \geq \frac{N}{\left(\sqrt{1 + \epsilon} - 1 \right)^2} = \left(\sqrt{1 + \epsilon} + 1 \right)^2\frac{N}{\epsilon^2}.
\]
\end{corollary}
\begin{proof}
Let $\epsilon$ and (even) integer $N \geq 2$ and vectors $u_1, \dots, u_m$ from Theorem~\ref{thm:harvey} be given, and pick $r$ satisfying the inequality in the theorem.
Thus by the previous corollary, there exists a partition $\{ A_1, \dots, A_r \}$ of $[m]$ so that 
\[
\norm{\sum_{i \in A_j} u_i u_i ^*} 
\leq \left(\frac{1}{\sqrt{r}}+\frac{1}{\sqrt{N}}\right)^{2}
\leq \frac{1 + \epsilon}{N}
\]
for all $j$ (as required). 
\end{proof}
In particular, $r \geq 6N / \epsilon^2$ suffices for $\epsilon < 1$.
Picking $N = 2$ and propagating this back through the arguments in \cite{harvey} gives Theorem~\ref{thm:anderson}.
%\end{document}
